Efficient Error-Tolerant Quantized Neural Network Accelerators

Neural Networks are currently one of the most widely deployed machine learning algorithms. In particular, Convolutional Neural Networks (CNNs), are gaining popularity and are evaluated for deployment in safety critical applications such as self driving vehicles. Modern CNNs feature enormous memory bandwidth and high computational needs, challenging existing hardware platforms to meet throughput, latency and power requirements. Functional safety and error tolerance need to be considered as additional requirement in safety critical systems. In general, fault tolerant operation can be achieved by adding redundancy to the system, which is further exacerbating the computational demands. Furthermore, the question arises whether pruning and quantization methods for performance scaling turn out to be counterproductive with regards to fail safety requirements. In this work we present a methodology to evaluate the impact of permanent faults affecting Quantized Neural Networks (QNNs) and how to effectively decrease their effects in hardware accelerators. We use FPGA-based hardware accelerated error injection, in order to enable the fast evaluation. A detailed analysis is presented showing that QNNs containing convolutional layers are by far not as robust to faults as commonly believed and can lead to accuracy drops of up to 10%. To circumvent that, we propose two different methods to increase their robustness: 1) selective channel replication which adds significantly less redundancy than used by the common triple modular redundancy and 2) a fault-aware scheduling of processing elements for folded implementations

==> experimental.tex <==
%\section{Experimental setup}
\section{Hardware Acceleration Results}
\label{sec:experimental}

To accelerate the experiments, we implemented the error injection simulation on a Xilinx ZCU104 board (XCZU7EV) running at 300 MHz. 
By scaling the folding factors, we were able to achieve 32,880 frames per second for the CNV-W1A1 and CNV-W1A2 topology on CIFAR-10 images. The CNV-W2A2 reached 20,833 FPS and W4A4 10,416 FPS.
With that, the evaluation of a complete whole channel stuck-at campaign for W1A1 containing 3,840 experiments was completed in 19 minutes. 
This is 5.8x faster than running Theano using a NVIDIA P40 where the overall campaign took 110 minutes.r The same campaign but evaluating for W1A2 and W2A2 required 5,760 experiments as 3 activation stages need to be injected. This took about 29 minutes for W1A2 and 46 minutes for W2A2 which is still an acceleration of 3.3x.
While the pixel stuck-at analysis requires a much larger amount of experiments, the runtime increases massively. The hardware acceleration allows to finish the experiments, only for layer 0 of CNV-W1A1 network, in about 15 hours, while the GPU solution requires approximately 87 hours.


==> tables/folding_factors_cnv.tex <==
\begin{table}[!ht]
\caption{folding factors used in the experiments for CNV network}\label{tab:nf-networks}
\resizebox{\columnwidth}{!}{ 
\begin{tabular}{c|c|cc|cc|cc|cc}
\multicolumn{2}{c}{}  & \multicolumn{2}{|c|}{cnv-W1A1} & \multicolumn{2}{|c|}{cnv-W1A2} & \multicolumn{2}{|c|}{cnv-W2A2} & \multicolumn{2}{|c}{cnv-W4A4}\\ \hline
layer & channels & PE      & SIMD    & PE   & SIMD & PE   & SIMD & PE   & SIMD \\ \hline
0 &  64 & 64 &   3 & 64 &    3 & 32 &   3 & 64 &   3\\
1 &  64 & 64 &  32 & 64 &   32 & 32 &  32 & 64 &   16\\
2 & 128 & 32 &  32 & 32 &   32 & 32 &  16 & 32 &   16\\
3 & 128 & 32 &  32 & 32 &   32 & 32 &  16 & 32 &   16\\
4 & 256 &  8 &  32 &  8 &   32 &  8 &  16 &  8 &   16\\
5 & 256 &  2 &  32 &  2 &   32 &  2 &  16 &  2 &   16\\
6 & 512 &  2 &   8 &  2 &    8 &  1 &   8 &  1 &    8\\
7 & 512 &  1 &  32 &  1 &   32 &  1 &  16 &  2 &    8\\
\end{tabular}
}
\end{table}

==> tables/folding_factors_lfc.tex <==
\begin{table}[!ht]
\caption{folding factors used in the experiments for LFC network, each PE computes NF (neuron fold) channels}\label{tab:nf-lfc}
\resizebox{\columnwidth}{!}{ 
\begin{tabular}{c|c|cc|cc|cc}
\multicolumn{2}{c}{}  & \multicolumn{2}{|c|}{lfc-W1A1} & \multicolumn{2}{|c|}{lfc-W1A2} & \multicolumn{2}{|c}{lfc-W2A2} \\ \hline
layer & channels & PE      & SIMD    & PE   & SIMD & PE   & SIMD \\ \hline
0 &  1024 & 32 & 64 & 32 &   64 & 16 &  16 \\
1 &  1024 & 64 & 64 & 64 &   64 & 16 &  32 \\
2 &  1024 & 64 & 64 & 64 &   64 & 16 &  32 \\

\end{tabular}
}
\end{table}

==> tables/sat-lfc-W1A1.tex <==
\begin{table}[t]
\caption{stuck-at for LFC-W1A1 network on MNIST}\label{tab:sat-lfc-W1A1}
\resizebox{\columnwidth}{!}{ 
\begin{tabular}{c|c|ccc|ccc}
\multicolumn{2}{c|}{} & \multicolumn{6}{c}{Accuracy in \%}\\
\multicolumn{2}{c|}{}  & \multicolumn{3}{c|}{stuck-at 0} & \multicolumn{3}{c}{stuck-at 1}     \\ \hline
layer & channels & min  & max & avg & min   & max & avg    \\ \hline
0 & 1024   & \textbf{98.39} & 98.52 & 98.46  & \textbf{98.39} & \textbf{98.53} & 98.46 \\
1 & 1024   & 98.42 & 98.51 & 98.46  & 98.41 & 98.50 & 98.46 \\
2 & 1024   & 98.46 & 98.47 & 98.47  & 98.46 & 98.47 & 98.47 
\end{tabular}
}
\vspace{-0.4cm}
\end{table}

==> tables/sat-lfc-W1A2.tex <==
\begin{table}[!ht]
\caption{stuck at faults in the LFC-W1A2 network for the MNIST dataset}\label{tab:sat-lfc-W1A2}
\resizebox{\columnwidth}{!}{ 
\begin{tabular}{c|c|ccc|ccc|ccc}
\multicolumn{2}{c}{values in \%}  & \multicolumn{3}{|c|}{stuck-at 1} & \multicolumn{3}{c}{stuck-at 0}  & \multicolumn{3}{c}{stuck-at -1}   \\ \hline
layer & channels & avg      & min    & max   & avg   & min   & max   & avg   & min   & max \\ \hline
0     & 1024     & 98.40    & 98.51  & 98.46 & 98.41 & 98.49 & 98.45 & 98.41 & 98.51 & 98.46 \\
1     & 1024     & 98.42    & 98.49  & 98.45 & 98.42 & 98.47 & 98.44 & 98.42 & 98.49 & 98.45 \\
2     & 1024     & 98.43    & 98.45  & 98.44 & 98.44 & 98.45 & 98.45 & 98.43 & 98.45 & 98.44
\end{tabular}
}
\end{table}

==> tables/sat-lfc-W2A2.tex <==
\begin{table}[!ht]
\caption{stuck at faults in the LFC-W2A2 network for the MNIST dataset}\label{tab:sat-lfc-W2A2}
\resizebox{\columnwidth}{!}{ 
\begin{tabular}{c|c|ccc|ccc|ccc}
\multicolumn{2}{c}{values in \%}  & \multicolumn{3}{|c|}{stuck-at 1} & \multicolumn{3}{c}{stuck-at 0}  & \multicolumn{3}{c}{stuck-at -1}   \\ \hline
layer & channels & avg      & min    & max   & avg   & min   & max   & avg   & min   & max \\ \hline
0 & 1024 & 98.52 & 98.46 & 98.55 & 98.51 & 98.46 & 98.55 & 98.52 & 98.44 & 98.57 \\
1 & 1024 & 98.52 & 98.48 & 98.55 & 98.53 & 98.50 & 98.55 & 98.52 & 98.48 & 98.55 \\
2 & 1024 & 98.53 & 98.51 & 98.54 & 98.53 & 98.52 & 98.53 & 98.53 & 98.51 & 98.54
\end{tabular}
}
\end{table}

==> tables/satchannel-cnv-W1A1.tex <==
\begin{table}[t]
\caption{whole channel stuck-at for CNV-W1A1 network on Cifar-10}\label{tab:satchannel-cnv-W1A1}
\centering
\resizebox{\columnwidth}{!}{ 
\begin{tabular}{c|c|ccc|ccc}
\multicolumn{2}{c|}{} & \multicolumn{6}{c}{Accuracy in \%} \\
\multicolumn{2}{c|}{}  & \multicolumn{3}{c|}{stuck-at 0} & \multicolumn{3}{c}{stuck-at 1}     \\ \hline
layer & channels & min & max & avg  & min & max & avg   \\ \hline
0 & 64 & 75.45 & \textbf{79.76} & 78.93 & 77.39 & 79.69 & 79.02 \\
1 & 64 & 77.57 & 79.25 & 78.75 & \textbf{73.01} & 79.26 & 77.24 \\
2 & 128 & 75.30 & 79.58 & 78.55 & 74.08 & 79.61 & 78.26 \\
3 & 128 & 78.08 & 79.36 & 78.89 & 76.23 & 79.23 & 78.13 \\
4 & 256 & 78.04 & 79.46 & 78.94 & 78.04 & 79.48 & 78.97 \\
5 & 256 & 78.85 & 79.43 & 79.17 & 78.84 & 79.40 & 79.18 \\
6 & 512 & 79.06 & 79.39 & 79.23 & 79.08 & 79.39 & 79.23 \\
7 & 512 & 79.16 & 79.29 & 79.23 & 79.17 & 79.29 & 79.23

\end{tabular}
}
\vspace{-0.5cm}
\end{table}

==> tables/satchannel-cnv-W1A2.tex <==
\begin{table}[!ht]
\caption{whole channel stuck-at for CNV-W1A2 network on Cifar-10}\label{tab:satchannel-cnv-W1A2}
\centering
\resizebox{\columnwidth}{!}{ 
\begin{tabular}{c|c|ccc|ccc|ccc}
\multicolumn{2}{c|}{} & \multicolumn{9}{c}{Accuracy in \%} \\
\multicolumn{2}{c|}{}  & \multicolumn{3}{c|}{stuck-at -1} & \multicolumn{3}{c|}{stuck-at 0} & \multicolumn{3}{c}{stuck-at 1} \\ \hline
layer & channels & min   & max   & avg   & min   & max   & avg   & min   & max   & avg  \\ \hline
0 & 64 & 80.82 & 83.11 & 82.53 & 81.76 & 83.11 & 82.57 & 79.43 & 82.93 & 82.37     \\
1 & 64 & 75.36 & 82.53 & 80.02 & 80.96 & 82.72 & 82.15 & 79.94 & \textbf{83.24} & 82.24    \\
2 & 128 & \textbf{71.85} & 83.03 & 81.10  & 79.91 & 83.18 & 82.21 & 73.81 & 82.98 & 81.54  \\
3 & 128  & 76.12 & 82.81 & 80.22 & 81.11 & 82.82 & 82.27 & 80.07 & 82.92 & 82.47  \\
4 & 256  & 80.57 & 82.81 & 82.25 & 82.03 & 82.83 & 82.47 & 80.52 & 82.84 & 82.29   \\
5 & 256  & 82.32 & 82.90 & 82.64 & 82.47 & 82.87 & 82.66 & 82.43 & 82.87 & 82.65   \\
6 & 512  & 82.53 & 82.88 & 82.69 & 82.57 & 82.81 & 82.69 & 82.49 & 82.83 & 82.68  \\
7 & 512  & 82.61 & 82.74 & 82.68 & 82.63 & 82.74 & 82.68 & 82.61 & 82.75 & 82.68 
\end{tabular}
}
\vspace{-0.6cm}
\end{table}

==> tables/satchannel-cnv-W2A2.tex <==
\begin{table}[!ht]
\caption{whole channel stuck-at for CNV-W2A2 network on Cifar-10}\label{tab:satchannel-cnv-W2A2}
\centering
\resizebox{\columnwidth}{!}{ 
\begin{tabular}{c|c|ccc|ccc|ccc}
\multicolumn{2}{c|}{}  & \multicolumn{9}{c}{Accuracy in \%}\\
\multicolumn{2}{c|}{}  & \multicolumn{3}{c|}{stuck-at -1} & \multicolumn{3}{c|}{stuck-at 0} & \multicolumn{3}{c}{stuck-at 1} \\ \hline
layer & channels & min & max & avg & min & max & avg & min & max & avg \\ \hline
0 & 64 & 82.62 & 84.45 & 84.01 & 83.48 & 84.69 & 84.17 & 80.50 & 84.68 & 83.90         \\
1 & 64 & 76.64 & 84.35 & 81.56 & 82.60 & 84.42 & 83.81 & 81.63 & 84.53 & 83.73         \\
2 & 128 & \textbf{74.18} & \textbf{84.76} & 82.62 & 82.44 & 84.56 & 83.76 & 74.80 & 84.59 & 83.05         \\
3 & 128  & 77.95 & 84.46 & 81.77 & 83.08 & 84.44 & 83.84 & 82.51 & 84.55 & 84.12        \\
4 & 256 & 81.52 & 84.63 & 83.96 & 83.74 & 84.65 & 84.22 & 82.54 & 84.53 & 84.02         \\
5 & 256 & 84.08 & 84.46 & 84.28 & 84.13 & 84.46 & 84.28 & 84.07 & 84.47 & 84.27         \\
6 & 512 & 84.12 & 84.45 & 84.28 & 84.15 & 84.45 & 84.29 & 84.09 & 84.46 & 84.28         \\
7 & 512 & 84.21 & 84.35 & 84.29 & 84.23 & 84.34 & 84.29 & 84.22 & 84.37 & 84.29        
\end{tabular}
}
%\vspace{-0.1cm}
\end{table}

==> tables/satchannel-cnv-W4A4.tex <==

\begin{table*}[!ht]
\caption{stuck at faults for a whole channel in the CNV-W4A4 network for the Cifar10 dataset}\label{tab:satchannel-cnv-W4A4}
\centering
\begin{adjustbox}{scale=0.8, angle=90}
\begin{tabular}{c|c|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc|ccc}
\multicolumn{2}{c}{values in \%}  & \multicolumn{3}{|c|}{stuck-at -4} & \multicolumn{3}{c|}{stuck-at -3} & \multicolumn{3}{c|}{stuck-at -2} & \multicolumn{3}{c|}{stuck-at -1} & \multicolumn{3}{c|}{stuck-at 0} & \multicolumn{3}{c|}{stuck-at 1} & \multicolumn{3}{c|}{stuck-at 2} & \multicolumn{3}{c|}{stuck-at 3} & \multicolumn{3}{c}{stuck-at 4} \\ \hline
layer & channels & avg & min & max & avg & min & max & avg & min & max & avg & min & max & avg & min & max & avg & min & max & avg & min & max & avg & min & max & avg & min & max \\ \hline
0 & 64 & 84.77 & 84.04 & 85.12 & 84.77 & 84.04 & 85.12 & 84.77 & 84.04 & 85.12 & 84.78 & 84.02 & 85.15 & 84.78 & 84.01 & 85.13 & 84.77 & 84.01 & 85.15 & 84.78 & 84.04 & 85.10 & 84.77 & 84.03 & 85.09 & 84.77 & 84.05 & 85.08 \\
1 & 64 & 84.42 & 82.25 & 85.16 & 84.60 & 83.23 & 84.92 & 84.69 & 83.82 & 85.22 & 84.62 & 83.44 & 84.98 & 84.46 & 82.72 & 85.06 & 84.16 & 81.80 & 84.89 & 83.73 & 80.23 & 84.87 & 83.14 & 78.69 & 84.70 & 82.44 & 77.00 & 84.76 \\
2 & 128 & 83.72 & 77.26 & 85.02 & 84.05 & 79.48 & 85.04 & 84.28 & 81.06 & 85.16 & 84.39 & 82.41 & 85.04 & 84.37 & 82.44 & 85.06 & 84.26 & 80.80 & 85.04 & 84.04 & 78.81 & 85.03 & 83.73 & 76.35 & 85.15 & 83.29 & 73.38 & 85.04 \\
3 & 128 & 84.64 & 82.09 & 84.99 & 84.73 & 82.86 & 85.02 & 84.69 & 83.41 & 85.03 & 84.55 & 83.72 & 84.93 & 84.27 & 82.86 & 84.87 & 83.86 & 81.57 & 84.89 & 83.32 & 79.71 & 84.88 & 82.62 & 77.84 & 84.89 & 81.79 & 75.48 & 85.09 \\
4 & 256 & 84.55 & 83.09 & 85.12 & 84.62 & 83.53 & 85.04 & 84.67 & 83.86 & 85.01 & 84.70 & 84.10 & 85.04 & 84.71 & 84.21 & 85.04 & 84.69 & 84.01 & 85.03 & 84.65 & 83.50 & 85.06 & 84.59 & 83.05 & 85.01 & 84.51 & 82.59 & 85.04 \\
5 & 256 & 84.83 & 84.60 & 84.99 & 84.84 & 84.60 & 85.00 & 84.85 & 84.67 & 84.99 & 84.85 & 84.65 & 85.01 & 84.85 & 84.66 & 84.98 & 84.85 & 84.62 & 84.99 & 84.84 & 84.62 & 84.97 & 84.84 & 84.60 & 85.00 & 84.83 & 84.59 & 85.00 \\
6 & 512 & 84.85 & 84.70 & 85.01 & 84.85 & 84.70 & 84.99 & 84.85 & 84.70 & 84.96 & 84.85 & 84.71 & 84.95 & 84.85 & 84.75 & 84.96 & 84.85 & 84.72 & 84.95 & 84.85 & 84.70 & 84.96 & 84.85 & 84.68 & 84.98 & 84.85 & 84.67 & 84.97 \\
7 & 512 & 84.86 & 84.78 & 84.92 & 84.86 & 84.80 & 84.92 & 84.86 & 84.81 & 84.91 & 84.86 & 84.81 & 84.92 & 84.86 & 84.82 & 84.92 & 84.86 & 84.82 & 84.91 & 84.86 & 84.81 & 84.91 & 84.86 & 84.81 & 84.93 & 84.86 & 84.79 & 84.93 
\end{tabular}
\end{adjustbox}
\end{table*}



==> tables/satpixel-cnv-W1A1.tex <==
%\begin{table}[!ht]
%\caption{stuck at faults for a single pixel in the cnv network for the cifar10 dataset}\label{tab:satpixel-cnv-W1A1}
%\centering
%\resizebox{\columnwidth}{!}{ 
%\begin{tabular}{c|cc|cc|c}
%\multicolumn{1}{c}{values in \%}  & \multicolumn{2}{|c|}{stuck-at 1} & \multicolumn{2}{c|}{stuck-at 0} & \multicolumn{1}{c}{}   \\ \hline
%layer & avg & min & avg & min  & \# faults per stuck-at\\ \hline
%0   & 78.47    & 77.85   & 78.47  & 77.69  & 57600 \\ 
%1   & 78.43    & 77.65   & 78.52  & 78.30  & 50176 (12544)  \\ 
%2   & 78.46    & 77.85   & 78.46  & 77.74  & 18432  \\ 
%3   & 78.45    & 77.96   & 78.52  & 78.37  & 12800 (3200)   \\ 
%4   & 78.49    & 78.11   & 78.49  & 78.11  & 2304       \\
%5   & 78.46    & 78.15   & 78.46  & 78.23  & 0   \\ 
%6   & 78.50    & 78.33   & 78.50  & 78.32  & 0  \\ 
%7   & 78.52    & 78.42   & 78.52  & 78.42  & 0
%\end{tabular}
%}
%\end{table}
\begin{table}[!ht]
\caption{single pixel stuck-at for CNV-W1A1 network on Cifar-10}\label{tab:satpixel-cnv-W1A1}
\centering
%\resizebox{\columnwidth}{!}{ 
\begin{tabular}{c|cc|cc}
                      & \multicolumn{4}{c}{Accuracy in \%}\\
\multicolumn{1}{c|}{} & \multicolumn{2}{c|}{stuck-at 0} & \multicolumn{2}{c}{stuck-at 1}   \\ \hline
layer & avg & min & avg & min \\  \hline
0   & 78.47  & \textbf{77.69} & 78.47    & 77.85    \\ 
1   & 78.52  & 78.30 & 78.43    & 77.65    \\ 
2   & 78.46  & 77.74 & 78.46    & 77.85     \\ 
3   & 78.52  & 78.37 & 78.45    & 77.96     \\ 
4   & 78.49  & 78.11 & 78.49    & 78.11   \\
5   & 78.46  & 78.23 & 78.46    & 78.15     \\ 
6   & 78.50  & 78.32 & 78.50    & 78.33     \\ 
7   & 78.52  & 78.42 & 78.52    & 78.42   
\end{tabular}
%}
\vspace{-0.5cm}
\end{table}
